Multicast Transmission Design with Enhanced DoF for MIMO Coded Caching Systems

Integrating coded caching (CC) into multi-input multi-output (MIMO) setups significantly enhances the achievable degrees of freedom (DoF). We consider a cache-aided MIMO configuration with a CC gain $t$, where a server with $L$ Tx-antennas communicates with $K$ users, each equipped with $G$ Rx-antennas. Similar to existing works, we also extend a core CC approach, designed initially for multi-input single-output (MISO) scenarios, to the MIMO setup. However, in the proposed MIMO strategy, rather than replicating the transmit scheme from the MISO setup, the number of users $\Omega$ served in each transmission is fine-tuned to maximize DoF. As a result, an optimized DoF of ${\max_{\beta, \Omega }}{\Omega \beta}$ is achieved, where ${\beta \le \mathrm{min}\big(G,L \binom{\Omega-1}{t}}\Big/{1 + (\Omega - t-1)\binom{\Omega-1}{t}}\big)$ is the number of parallel streams decoded by each user. For the considered MIMO-CC setup, we also introduce an effective multicast transmit covariance matrix design for the symmetric rate maximization objective solved iteratively via successive convex approximation (SCA). Finally, numerical simulations verify the enhanced DoF and improved performance of the proposed design.

==> Data/CCMAC.tex <==
SNR	B10OPT	B5OPT	B2OPT	B1OPT	B10toB1OPT	B2toB1OPT	B5toB1OPT
0	3.019496031	3.237992628	3.050747707	2.928696004	3 	4 	11 
5	6.006190989	6.203754341	5.843921052	5.537773058	8 	6 	12 
10	10.05986468	10.15248871	9.617257408	9.103326084	11 	6 	12 
15	15.12031657	15.05797721	14.20208891	13.39369048	13 	6 	12 
20	21.17906799	20.85934331	19.47841259	18.23805437	16 	7 	14 
25	27.93463344	27.3101688	25.33555066	23.39801623	19 	8 	17 
30	35.03084845	34.15059121	31.62450906	28.8261219	22 	10 	18 


==> Data/CCMC.tex <==
SNR	P15OPT	P12OPT	P6OPT	P3OPT	P15toP3OPT	P12toP3OPT	P6toPeOPT
0	3.019496031	2.942123949	2.24876639	2.042137213	48 	44 	10 
5	6.006190989	5.682989345	4.483561279	4.064630863	48 	40 	10 
10	10.05986468	9.36986002	7.625063013	6.907223017	46 	36 	10 
15	15.12031657	14.05027524	11.79554043	10.66633933	42 	32 	11 
20	21.17906799	19.84333005	17.17364819	15.52134839	36 	28 	11 
25	27.93463344	26.57432536	23.62563627	21.43007544	30 	24 	10 
30	35.03084845	33.78025068	30.73168825	28.10399695	25 	20 	9 


==> Data/CCMUX.tex <==
SNR	t2OPT	t1OPT	t0OPT	t2tot0OPT	t1tot0OPT	t2tot0TH	t1tot0TH
0	3.019496031	2.545210477	1.722927977	75 	48 	50 	25 
5	6.006190989	4.816306824	3.158179176	90 	53 	50 	25 
10	10.05986468	7.888027322	5.013348108	101 	57 	50 	25 
15	15.12031657	11.82856724	7.360721638	105 	61 	50 	25 
20	21.17906799	16.6813452	10.32663768	105 	62 	50 	25 
25	27.93463344	22.24682991	13.92519769	101 	60 	50 	25 
30	35.03084845	28.16252698	18.02488853	94 	56 	50 	25 


==> Data/SBF.tex <==
SNR	A4OPT	A3OPT	A2OPT	A1OPT	A4toA1OPT	A3toA1OPT	A2toA1OPT	A4toA1TH	A3toA1TH	A2toA1TH
0	3.019496031	3.255389193	3.19462742	3.03884808	-1 	7 	5 	100 	67 	33 
5	6.006190989	6.344362273	6.195238781	5.633862543	7 	13 	10 	100 	67 	33 
10	10.05986468	10.54495756	10.12109494	8.766504708	15 	20 	15 	100 	67 	33 
15	15.12031657	15.68325763	14.54256121	12.12092439	25 	29 	20 	100 	67 	33 
20	21.17906799	21.33266891	19.13520889	15.54965486	36 	37 	23 	100 	67 	33 
25	27.93463344	27.14877531	23.76366594	19.00050556	47 	43 	25 	100 	67 	33 
30	35.03084845	32.9969125	28.39100504	22.45708665	56 	47 	26 	100 	67 	33 
35

==> Data/SMUX.tex <==
SNR	L4OPT	L3OPT	L2OPT	L1OPT	L4toL1OPT	L3toL1OPT	L2toL1OPT	L4toL1TH	L3toL1TH	L2toL1TH	L4toL3OPT	L4toL3TH	L4toL2OPT	L4toL2TH
0	3.019496031	2.49186387	1.423904776	0.597396735	405 	317 	138 	100 	67 	33 	21 	20 	112 	50 
5	6.006190989	5.008934723	3.162012335	1.512479737	297 	231 	109 	100 	67 	33 	20 	20 	90 	50 
10	10.05986468	8.497909094	5.709079172	3.223654597	212 	164 	77 	100 	67 	33 	18 	20 	76 	50 
15	15.12031657	12.96424947	8.899232124	5.738082738	164 	126 	55 	100 	67 	33 	17 	20 	70 	50 
20	21.17906799	18.26457795	12.76218425	8.807504004	140 	107 	45 	100 	67 	33 	16 	20 	66 	50 
25	27.93463344	24.06475332	17.17230996	12.16160646	130 	98 	41 	100 	67 	33 	16 	20 	63 	50 
30	35.03084845	30.04428564	21.91653976	15.63077287	124 	92 	40 	100 	67 	33 	17 	20 	60 	50 
35

==> Data/STYPE.tex <==
SNR	L4A4OPT	L4A4ZF	L4A2OPT	L4A2ZF	L4A4OPTtoZF	L4A2OPTtoZF
0	3.019496031	0.442695864	3.19462742	1.76642666	582 	81 
5	6.006190989	1.342893157	6.195238781	4.218965827	347 	47 
10	10.05986468	3.768993242	10.12109494	8.022700117	167 	26 
15	15.12031657	8.9253664	14.54256121	12.54641351	69 	16 
20	21.17906799	16.63372103	19.13520889	17.25074781	27 	11 
25	27.93463344	25.62381906	23.76366594	21.94334747	9 	8 
30	35.03084845	34.2407576	28.39100504	26.6036158	2 	7 


==> Figs/data.tex <==
SNR	RsymLG22K3t1	RsymLG22K2t1Icasp	RsymLG22K2t1logdet	RsymLG42K3t1	RsymLG42K4t1	RsymLG42K5t1	RsymLG32K3t1	    RsymLG32K4t1	RsymLG32K2t1	RsymLG22K4t2	RsymLG22K3t2	RsymLG44K3t2	RsymLG42K4t2	RsymLG42K5t2		RsymLG42K3t1WSAZFUnicast				RsymLG32K2t1WSAZFUnicast				RsymLG33K2t1CovMC			RsymLG33K2t1ICASSPMC			RsymLG42K2t0MIMOUnicast			RsymLG42K3t0MIMOUnicast	
																																		
0	3.7593	3.5884	3.6949	6.368	6.4835	6.4895	5.3364	5.3014	4.8047	5.1351	5.599797754	13.34196235	9.4370082	9.689970023			2.970622533			2.143022131				6.1049			4.614377371				3.609143706			3.831366754
5	7.3608	6.6367	6.811	11.9051	12.2979	12.1508	10.1282	10.105	8.6826	10.2022	10.61654854	24.35043282	18.0546017	18.55265585			6.438479039			4.420501449				11.0308			7.742104821				6.389178313			7.146762946
10	12.3646	10.88	11.0363	19.3557	19.88	19.2401	16.5233	16.6818	14.0075	17.391	17.45430476	39.31712964	29.77676128	30.25348613			12.0213435			7.885372607				17.6536			12.11221205				9.940045125			11.45468669
15	18.0988	16.2032	16.3266	28.3209	28.2528	28.9142	24.0291	24.1823	20.4462	25.7781	25.97294365	57.41497012	43.77187859	43.22326524			19.9216751			12.67259089				25.7262			18.57064199				14.21201437			16.27030372
20	23.9393	22.4398	22.5407	38.3617	36.6317	38.3004	32.4269	31.8489	27.4743	34.332	36.05074603	77.9366746	59.17270754	56.25538893			29.5694723			18.62366488				34.9933			27.07585974				19.20715816			21.24552112
25	29.7181	29.2683	29.3885	49.019	44.6427	47.5525	41.6848	39.3423	34.7368	42.5595	47.35962381	100.3251136	75.28520935	68.480869			40.10652076			25.34656728				45.0972			36.92470546				25.01281006			26.15783114
30	35.0913	36.408	36.561	59.945	52.3203	56.4409	51.6823	46.5181	42.0801	49.9784	59.3550591	123.9490157	91.70442413	79.98266217			50.99824058			32.45275667				55.7393			47.45136196				30.94294126			30.99439917


==> Figs/data_Globcom.tex <==
SNR 	RsymLG32K3t1ISITcov	 RsymLG32K3MMSESIC  RsymLG32K3MMSE
					
0	5.3365	5.1562   4.2877
5	10.1285	9.6274 	7.5527
10	16.5253	15.5328	 12.4468
15	24.0321	22.4945	 18.6496
20	32.4362	30.2347	 25.7339
25	41.6948	38.6218	 33.8356
30	51.7005	47.4762	 42.7128


==> Transmission_Strategy.tex <==
% %Here we provide examples of how the transmission user target size affects the problem and what we expect in each case on the covariance matrix rank behavior.
% In this section, we analyze the impact of various multigroup multicast transmission configurations and reveal how the chosen transmission strategy can influence both the MIMO-CC system design and its performance. We assume a content delivery scenario illustrated in Fig.1, where a transmitter with $L$ antennas should fulfill requests from $K = 10$ users, each equipped with $G =2$ antennas.
% We compute the symmetric rate $R_{sym}$ in \eqref{eq:TX_signal}, taking into account the number of transmission vectors and codeword lengths, while assuming the same content placement strategy as in~\cite{maddah2014fundamental}.  It should be noted that, as discussed in Section~\ref{section:sys_model}, we need to further split each subfile $W_{\CP}$ into $\binom{K-t-1}{\Omega-t-1}$ smaller chunks $W_{\CP}^q$. However, as a matter of simplicity, chunk indices $q$ are ignored here since they do not have any influence on the algorithm's behavior. Moreover, throughout this analysis, we focus on the transmission vector in a single time slot, even though the data transfer takes place over multiple consecutive time slots (in each slot, $\Omega$ users are served). Below, we illustrate various configurations through a number of examples to provide a better understanding.
% %Here, we examine the configuration of multigroup multicast transmissions for various setups, and illustrate how the size of the transmission target affects the problem.
% %We consider multigroup multicast covariance matrix design for different setups explained in various examples.  
% %\subsection{Scenario 1: $L \geq 3$, $G = 2$, and $t=1$} 
% %\subsubsection{ $|\CK| = 3$ Selected User Served }

\begin{exmp}
    \label{exmp:x3serv}
\normalfont
In this example, the BS has $L=4$ antennas and serves  $\Omega = 3$ users, and the CC gain is $t = 1$ (i.e., $\textrm{DoF} =6$). For notational simplicity, let us assume that $ A$, $B$, and $C$ denote the files requested by users 1-3, respectively.
For this setup, the multicast transmission vector for users~1-3 can be written as
\begin{IEEEeqnarray}{lll}\label{eq:Psig}
		{\Bx}= {\Bx}_{1,2}   + {\Bx}_{1,3} + {\Bx}_{2,3},
	\end{IEEEeqnarray}
where each signal is proportional to its transmitted message, i.e., $ {\Bx}_{1,2} \propto (A_2\oplus B_1) $, $ {\Bx}_{1,3} \propto (A_3\oplus C_1)  $, $ {\Bx}_{2,3} \propto (B_3\oplus C_2) $.\footnote{As a special case, in~\eqref{eq:Psig}, we may use linear transmit precoders $ \Bw_{\mathcal{T}}$, defined by indices~$\mathcal{T} \in \{\{1,2\}, \{1,3\}, \{2,3\}\}$, to get the transmission vector
		${\Bx}= (A_2\oplus B_1)\Bw_{1,2} + (A_3\oplus C_1)\Bw_{1,3} + (B_3\oplus C_2) \Bw_{2,3}$~\cite{tolli2018multicast}.}
 
Then, the received signals at users 1-3 can be expressed as:
\begin{IEEEeqnarray}{lll}\label{eq:rx_sig}
		\By_1 = \underline{\BH_1 {\Bx}_{1,2}}   + \underline{\BH_1{\Bx}_{1,3}} + \BH_1 {\Bx}_{2,3} + \Bz_1\; ,\nonumber\\
  \By_2 = \underline{\BH_2 {\Bx}_{1,2}} + \underline{\BH_2 {\Bx}_{2,3}} + \BH_2{\Bx}_{1,3} + \Bz_2\; ,\\
  \By_3 = \underline{\BH_3 {\Bx}_{1,3}} + \underline{\BH_3 {\Bx}_{2,3}} + \BH_3{\Bx}_{1,2} + \Bz_3\;\nonumber ,
\end{IEEEeqnarray}
where underlined terms correspond to the desired signals for each user.
Now, if we consider user~1, both ${\Bx}_{1,2}$ and ${\Bx}_{1,3}$ are desired signals while
${\Bx}_{2,3}$ appears as Gaussian interference. Thus, $\By_1$ represents a Gaussian MAC channel, and user 1 can decode both of its required messages with the equal rate of
\begin{equation}
    R_{MAC}^1  = \text{min}\Big(R_{\{1,2\}}^{}, R_{\{1,3\}}^{}, \frac{1}{2} R_{{\{\{1,2\}, \{1,3\}\}}}^{}\Big),
\end{equation}
%$$,
where $R_{{\{\{1,2\}, \{1,3\}\}}}^{} = R_{\{1,2\}}^{} + R_{\{1,3\}}^{}$, and $R_{\{1,2\}}^{}$ and $R_{\{1,3\}}^{}$ correspond to ${\Bx}_{1,2}$ and ${\Bx}_{1,3}$, respectively. Using this example as a guide, $\CK  =\{1,2,3\}$, $\mathsf S^{\CK} = \{\{1,2\}, \{1,3\}, \{2,3\}\}$, $\mathsf S_1^{\CK}  = \{\{1,2\}, \{1,3\}\}$, $\bar{\mathsf S}_1^{\CK}  = \{\{2,3\}\}$, and $\mathsf B $ could be selected as $\{\{1,2\}\}$, $ \{\{1,3\}\}$, or $  \{\{1,2\}, \{1,3\}\}$.
 
Therefore, the optimum multicast transmission rate, determined w.r.t the covariance matrices $\mathbf{K}_{{\Bx}_{1,2}}$, $\mathbf{K}_{{\Bx}_{1,3}}$, $\mathbf{K}_{{\Bx}_{2,3}}$ can be found by solving~\eqref{eq:P_optimum2}
where $\BQ_{1}  =  N_0\mathbf{I}+\mathbf{H}_1 \mathbf{K}_{{\Bx}_{2,3}}\mathbf{H}_1^H $, $\BQ_{2}  =   N_0 \mathbf{I}+\mathbf{H}_2 \mathbf{K}_{{\Bx}_{1,3}}\mathbf{H}_2^H $, and $\BQ_{3}  =   N_0\mathbf{I}+\mathbf{H}_3 \mathbf{K}_{{\Bx}_{1,2}}\mathbf{H}_3^H $. The relevant Problem is nonconvex; however, it can be readily solved by the proposed SCA in \textbf{Algorithm 1}.
 \end{exmp}
\begin{exmp}\label{exmp:x5serv}
    \normalfont This example addresses the special case of $L=G$ and $\Omega = {t + 1}$ in Remark~\ref{remark1}.
    %, where the multicast signal vector ${\Bx}= {\Bx}_{1,2,3}$, 
    Assume $ \Omega  = 3$, and $t = 2 $ (for this configuration, $\textrm{DoF}=3 \times G$ for any $G$). Upon transmitting signal vector $\Bx = \Bx_{1,2,3}$, the received signal vectors are $\By_k = \BH_k {\Bx}_{1, 2, 3} + \Bz_k$. In this case, there is no interference and the optimal multicast rate solution is obtained by
\begin{equation}
\label{eq:P_optimum1_K1_symexm}
\begin{aligned}
&\max_{\mathbf{K}_{{\Bx}_{1, 2, 3}}, R_{}^k} \min_{k\in \CK} 
  (R_{}^1, R_{}^2, R_{}^3) \\
    &s.t.\quad R_{}^{k} \leq \log|\mathbf{I}+\mathbf{H}_k \mathbf{K}_{{\Bx}_{1, 2, 3}}\mathbf{H}_k^H|, \; \\
    & \quad\:\quad \text{Tr}(\mathbf{K}_{{\Bx}_{1, 2, 3}})
	  \leq P_T .
\end{aligned}
\end{equation}
where the convex problem~\eqref{eq:P_optimum1_K1_symexm} could be efficiently tackled with CVX solvers. 
\end{exmp}



==> wrapup.tex <==
For MISO-native parameters:
\begin{itemize}
    \item Having larger antenna arrays is always good as it adds a whole new resource to the system.
    \item For a fixed antenna array size, at the finite-SNR regime it is better to trade the spatial multiplexing gain with the beamformer directivity. Fortunately, this does not impose any structural changes to the underlying caching scheme, i.e., we do not need to design a new CC scheme. Moreover, it only affects the second-layer subpacketization (before the transmission), and hence, this parameter can be selected instantly and over the air. \textbf{This property should be kept in mind as we design new CC schemes.}
    \item As expected, optimized beamformers always outperform zero-forcing. However, the gap between the two strategies narrows down heavily at high-SNR. The gap can also be reduced at the finite-SNR regime by reducing the spatial MUX gain. So, reducing the spatial multiplexing gain at the finite-SNR regime has also another benefit: we can use less-complex ZF beamformers if complexity is a big issue.
    \item Designing less-complex optimized beamformer designs well-tailored for CC schemes is of much interest. One interesting work is done by Nariman in~\cite{mahmoodi2021low}. However, it only applies when the CC MAC size is one.
\end{itemize}

For CC-native parameters:
\begin{itemize}
    \item Similar to the antenna count, having more memory is always good as it adds a whole new resource to the system. There is one important difference, though: the gain from having more memory is less-dependent on the SNR and can be achieved regardless of the SNR value (which makes sense, as memory-aided interference cancellation has nothing to do with the SNR value).
    \item The CC multiplexing gain also plays an important role (up to 50\%) in the achievable performance. However, this is a tricky parameter to play with: on the one hand, we have pure signal-level CC schemes that provide lots of benefits such as handling dynamicity, reduced subpacketization, easy extension to MIMO setups, etc. and on the other hand are pure bit-level schemes that provide the highest multicasting gain and hence the highest possible performance. It is a big question whether this trade-off could be tuned more gently; i.e. whether we could have some benefits of the signal-level schemes while keeping at least part of the multicasting gain. For example, the easy beamformer design is shown to be doable for some bit-level schemes (Nariman), and reduced subpacketization is also shown to be possible somehow (Soheil and Itsik). A more thorough study is highly encouraged.
    \item Increasing the MAC size provides a very small benefit but adds much to the complexity. Specifically, it requires much more complex receivers. If removing the MAC makes bit-level schemes more flexible, e.g., by allowing simpler beamformer designs for them, we should aim for that.
\end{itemize}
